NR-SLAM: Non-Rigid Monocular SLAM

In this paper we present NR-SLAM, a novel non-rigid monocular SLAM system founded on the combination of a Dynamic Deformation Graph with a Visco-Elastic deformation model. The former enables our system to represent the dynamics of the deforming environment as the camera explores, while the later allows us to model general deformations in a simple way. The presented system is able to automatically initialize and extend a map modeled by a sparse point cloud in deforming environments, that is refined with a sliding-window Deformable Bundle Adjustment. This map serves as base for the estimation of the camera motion and deformation and enables us to represent arbitrary surface topologies, overcoming the limitations of previous methods. To assess the performance of our system in challenging deforming scenarios, we evaluate it in several representative medical datasets. In our experiments, NR-SLAM outperforms previous deformable SLAM systems, achieving millimeter reconstruction accuracy and bringing automated medical intervention closer. For the benefit of the community, we make the source code public.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> backup.tex <==
Deformable SLAM problem consists in reconstructing a map whose shape is constantly deforming and recovering the camera trajectory with respect to the reconstructed map. This is well know to be an ill-posed problem from which infinite solutions arise \cite{huang2021some}. In order to constrain all possible solutions to a reduced set of reasonable reconstructions, many authors address this problem using sensors that provide 3D information (i.e. pixel depths) to reduce the number of variables to solve. One of the most notable methods is DynamicFusion \cite{newcombe2015dynamicfusion} which proposes to use a RGB-D camera to get dense reconstructions from deformable scenes (people moving). Later, MIS-SLAM \cite{song2018mis} presented its own approach with stereo cameras in medical sequences by using ORB-SLAM \cite{mur2015orb} as a base algorithm to get rigid reconstructions to later apply deformable techniques. Another interesting work, while not being a 3D sensor is \cite{xue2022event} in which a stationary event camera is used to reconstruct deformable objects.

Other family of methods for deformable SLAM is the one that make use of a precomputed 3D model of the observed surface. \cite{collins2020augmented} uses a CT or MT of an organ to get an initial 3D estimation of the map that will be later used by a rigid SLAM. \cite{schule2022model} combines 3D model simulation with finite elements simulation and a SLAM algorithm to reconstruct simulated deformable surfaces. Finally, MORPH-DSLAM \cite{badias2021morph} uses CAD models to reconstruct scenes where there is an object that undergoes some deformations using monocular deformable SLAM. The main peculiarity of this method is the fact that they reduce the DoF of the deforming objects by modeling the physical possible deformations a known object can suffer. \cite{cui2021virtual} uses rigid SLAM to get a point cloud reconstruction from nasal endoscopy sequences that is later aligned with a CT 3D model.

A subproblem of deformable SLAM is SLAM in dynamic scenarios. The aim of this subproblem is to solve SLAM in scenarios where there are rigid objects that can move freely. DynaSLAM \cite{bescos2018dynaslam} uses neural networks to segment dynamic objects and remove them from the SLAM pipeline. The follow up work DynaSLAM II \cite{bescos2021dynaslam} uses stereo/RGB-D SLAM to compute the 3D pose of dynamic objects along with the static part of the map. DOT \cite{ballester2021dot} is a work similar to DynaSLAM II but it also introduces the use of dynamic object masks obtained with neural networks

With the boom of deep learning techniques, many authors decide to integrate deep learning techniques to solve the deformable SLAM problem. For example, E-DSSR \cite{long2021dssr} uses a transformer based network to compute depth from stereo images that, in conjunction with a surgical tool segmentation network. Endo-Depth-and-Motion \cite{recasens2021endo} uses a monocular depth network to reconstruct medical sequences using photometric SLAM. \cite{barbany2022deformable} proposes a neural network to reconstruct continous and dense surfaces from a template imposing preservation of the riemannian metric as loss function. \cite{liu2022sage} proposes a method that uses monocular depth networks along with a featuremetric Bundle Adjutment to solve the deformable reconstruction problem.

All methods mentioned until now make use of some type of 3D clue to solve (or at least constrain) the deformable SLAM problem in the form of 3D sensors or deep learning techniques. While those methods have been proven to work, they are not easy (or even possible) to use in real applications. For example, in medical sequences it is not possible to use stereo/RGB-D cameras due to size restrictions. Also the use of deep learning techniques can be tricky as it is hard to find enough labeled data or self-supervised strategies to train the models. For that reason, pure monocular deformable SLAM is needed for real world applications. The first system to tackle this problem is DefSLAM \cite{lamarca2020defslam}, which uses a combination of Non-Rigid Structure-from-Motion for mapping, and template-based techniques for tracking. Later, SD-DefSLAM \cite{gomez2021sd} incorporates on top of DefSLAM a photometric feature matching method to increase the accuracy and robustness of the algorithm. The main limitation of this family of algorithms is their inability to model surfaces with discontinuities or non-isometric deformations. To tackle that, \cite{lamarca2021direct} proposes a method to perform photometric camera and deformation tracking when an initial 3D estimation of the surface is available. This method is able to model surface discontinuities by representing the map as a set of sparse surfels that move independently. However, it still relies on an initial 3D estimation and the assumption of isometric surfaces. \cite{rodriguez2022tracking} presents a pure monocular algorithm for camera pose tracking and deformation estimation that does not rely in isometry. This allows this method to be applied to real medical sequences with different type of topologies and deformations. Finally, another method that is worth mentioning is \cite{zhou2021real}. This is a 2D deformable monocular SLAM used to build panoramas and mosaicking of medical sequences.

While solving the full deformable SLAM problem is the main focus of the research community, some authors decide to solve subproblems of deformable SLAM, mainly applied to medical use cases. For example, in \cite{batlle2022photometric}, authors propose a way to compute monocular depth in colonoscopies using differentiable rendering techniques. Some other authors explore the use of different combinations of feature-descriptors for medical SLAM like in \cite{oliva2022orb}, in which they modify ORB-SLAM3 \cite{campos2021orb}, incorporating image contrast improving techniques, AKAZE and SuperPoint features applied to uretersocopies. The work in \cite{wu20223d} also makes a similar study of contrast improvements and AKAZE features for laparoscopic sequences. \cite{wang2022monocular} studies the use of SIFT features for gastroscopy tracking and compares it with other hand-crafted features. Finally, the work presented in\cite{lin2022semantic}, while not being an SLAM system, proposes a deep learning framework that solves several tasks: monocular depth, semantic segmentation and tool tracking.

\textbf{¿Seria buena idea hacer una tabla comparativa de los diferentes metodos mencionados como hicimos en el ORB-SLAM? Un ejemplo rpaido seria la Tabla \ref{tab::related_work}.}

\textbf{Tambien podria ser buena idea poner un parrafo con las dificultades presentes al evaluar el SLAM deformable: muy pocos datasets y ninguno estandard (dificil de comparar), muchos son medicos que añaden dificultades extras, cada paper usa sus propias secuencias (muchas siendo simulaciones sin casos reales), falta de metricas standards y disponibilidad de groundtruth y etiquetas.}

One of the main problems in the research in deformable SLAM is the lack of standard datasets and labeled data. Most of the mentioned methods above use custom sequences recorded specifically for the work in which they are presented and are usually not publicly available. Moreover, some works make use of simulations that, while useful, they are over-simplifications of real use cases. One of the most used dataset is the Hamlyn dataset \cite{mountney2010three}, which is composed of several in-vivo and ex-vivo intracorporeal sequences. The main reason of the popularity of this dataset is that most sequences where recorded with a stereo endoscope which can be used to get a pseudo-groundtruth of the surfaces imaged. More recently the Endomapper dataset \cite{azagra2022endomapper} presented a dataset of calibrated colonoscopies. The main drawback of this dataset is the lack of lables/groundtruth as the colonospies are recorded with a monocular endoscope with no 3D groundtruth. To tackle this, the dataset also provides some simulated colononscopy sequences with both depthand camera pose groundtruth.

\begin{table}[]
\caption{Ejemplo de tabla para comparar el estado del arte (parecida a la del ORB-SLAM3).}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Method                                       & Sensor used                                                   & \begin{tabular}[c]{@{}c@{}}Is an SLAM \\ algorithm?\end{tabular} & \begin{tabular}[c]{@{}c@{}}Deformable \\ formulation?\end{tabular} & \begin{tabular}[c]{@{}c@{}}Uses \\ 3D clues?\end{tabular}           & \begin{tabular}[c]{@{}c@{}}Applied to \\ endoscopies?\end{tabular} \\ \hline
DefSLAM                                      & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & Yes                                                              & Yes                                                                & No                                                                  & Yes                                                                \\ \hline
SD-DefSLAM                                   & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & Yes                                                              & Yes                                                                & No                                                                  & Yes                                                                \\ \hline
MORPH-DSLAM                                  & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & Yes                                                              & Yes                                                                & \begin{tabular}[c]{@{}c@{}}CAD \\ model\end{tabular}                & No                                                                 \\ \hline
\cite{collins2020augmented} & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & Yes                                                              & Yes                                                                & \begin{tabular}[c]{@{}c@{}}CT-MT\\ model\end{tabular}               & Yes                                                                \\ \hline
Endo-Depth-and-Motion                        & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & Yes                                                              & No                                                                 & \begin{tabular}[c]{@{}c@{}}Depth from\\ neural network\end{tabular} & Yes                                                                \\ \hline
DynaSLAM                                     & \begin{tabular}[c]{@{}c@{}}Stereo/RGB-D\\ camera\end{tabular} & Yes                                                              & No                                                                 & \begin{tabular}[c]{@{}c@{}}Depth from \\ stereo/RGB-D\end{tabular}  & No                                                                 \\ \hline
Dynamic-Fusion                               & \begin{tabular}[c]{@{}c@{}}RGB-D \\ camera\end{tabular}       & Yes                                                              & Yes                                                                & \begin{tabular}[c]{@{}c@{}}Depth\\ from RGB-D\end{tabular}          & No                                                                 \\ \hline
MIS-SLAM                                     & \begin{tabular}[c]{@{}c@{}}Stereo\\ camera\end{tabular}       & Yes                                                              & Yes                                                                & \begin{tabular}[c]{@{}c@{}}Depth\\ from stereo\end{tabular}         & Yes                                                                \\ \hline
DSDT                                         & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & No                                                               & Yes                                                                & \begin{tabular}[c]{@{}c@{}}Initial depth\\ from stereo\end{tabular} & Yes                                                                \\ \hline
MCPD                                         & \begin{tabular}[c]{@{}c@{}}Monocular\\ camera\end{tabular}    & No                                                               & Yes                                                                & No                                                                  & Yes                                                                \\ \hline
\end{tabular}
\label{tab::related_work}
\end{table}

@article{collins2020augmented,
  title={Augmented reality guided laparoscopic surgery of the uterus},
  author={Collins, Toby and Pizarro, Daniel and Gasparini, Simone and Bourdel, Nicolas and Chauvet, Pauline and Canis, Michel and Calvet, Lilian and Bartoli, Adrien},
  journal={IEEE Transactions on Medical Imaging},
  volume={40},
  number={1},
  pages={371--380},
  year={2020},
  publisher={IEEE}
}

@inproceedings{schule2022model,
  title={A Model-based Simultaneous Localization and Mapping Approach for Deformable Bodies},
  author={Sch{\"u}le, Johannes and Haag, Jonathan and Somers, Peter and Veil, Carina and Tar{\'\i}n, Christina and Sawodny, Oliver},
  booktitle={2022 IEEE/ASME International Conference on Advanced Intelligent Mechatronics (AIM)},
  pages={607--612},
  year={2022},
  organization={IEEE}
}

@inproceedings{cui2021virtual,
  title={Virtual reality navigation system of nasal endoscopy with real surface texture information},
  author={Cui, Zhouhai and He, Yucheng and Zhang, Peng and Hu, Ying and Jin, Haiyang and Liu, Shoubin},
  booktitle={2021 IEEE International Conference on Real-time Computing and Robotics (RCAR)},
  pages={135--140},
  year={2021},
  organization={IEEE}
}

@article{badias2021morph,
  title={MORPH-DSLAM: Model Order Reduction for PHysics-based Deformable SLAM},
  author={Badias, Alberto and Alfaro, Iciar and Gonzalez, David and Chinesta, Francisco and Cueto, Elias},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
  publisher={IEEE}
}

@inproceedings{huang2021some,
  title={Some Research Questions for SLAM in Deformable Environments},
  author={Huang, Shoudong and Chen, Yongbo and Zhao, Liang and Zhang, Yanhao and Xu, Mengya},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={7653--7660},
  year={2021},
  organization={IEEE}
}

@article{song2018mis,
  title={Mis-slam: Real-time large-scale dense deformable slam system in minimal invasive surgery based on heterogeneous computing},
  author={Song, Jingwei and Wang, Jun and Zhao, Liang and Huang, Shoudong and Dissanayake, Gamini},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={4},
  pages={4068--4075},
  year={2018},
  publisher={IEEE}
}

@inproceedings{long2021dssr,
  title={E-dssr: efficient dynamic surgical scene reconstruction with transformer-based stereoscopic depth perception},
  author={Long, Yonghao and Li, Zhaoshuo and Yee, Chi Hang and Ng, Chi Fai and Taylor, Russell H and Unberath, Mathias and Dou, Qi},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={415--425},
  year={2021},
  organization={Springer}
}

@article{recasens2021endo,
  title={Endo-Depth-and-Motion: Reconstruction and tracking in endoscopic videos using depth networks and photometric constraints},
  author={Recasens, David and Lamarca, Jos{\'e} and F{\'a}cil, Jos{\'e} M and Montiel, JMM and Civera, Javier},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={4},
  pages={7225--7232},
  year={2021},
  publisher={IEEE}
}

@article{bescos2018dynaslam,
  title={DynaSLAM: Tracking, mapping, and inpainting in dynamic scenes},
  author={Bescos, Berta and F{\'a}cil, Jos{\'e} M and Civera, Javier and Neira, Jos{\'e}},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={4},
  pages={4076--4083},
  year={2018},
  publisher={IEEE}
}

@article{bescos2021dynaslam,
  title={DynaSLAM II: Tightly-coupled multi-object tracking and SLAM},
  author={Bescos, Berta and Campos, Carlos and Tard{\'o}s, Juan D and Neira, Jos{\'e}},
  journal={IEEE robotics and automation letters},
  volume={6},
  number={3},
  pages={5191--5198},
  year={2021},
  publisher={IEEE}
}

@inproceedings{ballester2021dot,
  title={DOT: Dynamic object tracking for visual SLAM},
  author={Ballester, Irene and Font{\'a}n, Alejandro and Civera, Javier and Strobl, Klaus H and Triebel, Rudolph},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={11705--11711},
  year={2021},
  organization={IEEE}
}

@article{zhou2021real,
  title={Real-time nonrigid mosaicking of laparoscopy images},
  author={Zhou, Haoyin and Jayender, Jagadeesan},
  journal={IEEE Transactions on Medical Imaging},
  volume={40},
  number={6},
  pages={1726--1736},
  year={2021},
  publisher={IEEE}
}

@article{lin2022semantic,
  title={Semantic-SuPer: A Semantic-aware Surgical Perception Framework for Endoscopic Tissue Classification, Reconstruction, and Tracking},
  author={Lin, Shan and Miao, Albert J and Lu, Jingpei and Yu, Shunkai and Chiu, Zih-Yun and Richter, Florian and Yip, Michael C},
  journal={arXiv preprint arXiv:2210.16674},
  year={2022}
}

@article{barbany2022deformable,
  title={Deformable Surface Reconstruction via Riemannian Metric Preservation},
  author={Barbany, Oriol and Colom{\'e}, Adri{\`a} and Torras, Carme},
  journal={arXiv preprint arXiv:2212.11596},
  year={2022}
}

@article{liu2022sage,
  title={SAGE: SLAM with Appearance and Geometry Prior for Endoscopy},
  author={Liu, Xingtong and Li, Zhaoshuo and Ishii, Masaru and Hager, Gregory D and Taylor, Russell H and Unberath, Mathias},
  journal={arXiv preprint arXiv:2202.09487},
  year={2022}
}

@article{batlle2022photometric,
  title={Photometric single-view dense 3D reconstruction in endoscopy},
  author={Batlle, Victor M and Montiel, Jos{\'e} MM and Tardos, Juan D},
  journal={arXiv preprint arXiv:2204.09083},
  year={2022}
}

@article{xue2022event,
  title={Event-based Non-Rigid Reconstruction from Contours},
  author={Xue, Yuxuan and Li, Haolong and Leutenegger, Stefan and St{\"u}ckler, J{\"o}rg},
  journal={arXiv preprint arXiv:2210.06270},
  year={2022}
}

@article{oliva2022orb,
  title={An ORB-SLAM3-based Approach for Surgical Navigation in Ureteroscopy},
  author={Oliva Maza, Laura and Steidle, Florian and Klodmann, Julian and Strobl, Klaus and Triebel, Rudolph},
  journal={Computer Methods in Biomechanics and Biomedical Engineering: Imaging \& Visualization},
  pages={1--7},
  year={2022},
  publisher={Taylor \& Francis}
}

@article{campos2021orb,
  title={Orb-slam3: An accurate open-source library for visual, visual--inertial, and multimap slam},
  author={Campos, Carlos and Elvira, Richard and Rodr{\'\i}guez, Juan J G{\'o}mez and Montiel, Jos{\'e} MM and Tard{\'o}s, Juan D},
  journal={IEEE Transactions on Robotics},
  volume={37},
  number={6},
  pages={1874--1890},
  year={2021},
  publisher={IEEE}
}

@article{wu20223d,
  title={3D Texture Reconstruction of Abdominal Cavity Based on Monocular Vision SLAM for Minimally Invasive Surgery},
  author={Wu, Haibin and Xu, Ruotong and Xu, Kaiyang and Zhao, Jianbo and Zhang, Yan and Wang, Aili and Iwahori, Yuji},
  journal={Symmetry},
  volume={14},
  number={2},
  pages={185},
  year={2022},
  publisher={MDPI}
}

@article{wang2022monocular,
  title={A monocular SLAM system based on SIFT features for gastroscope tracking},
  author={Wang, Yifan and Zhao, Liang and Gong, Lun and Chen, Xin and Zuo, Siyang},
  journal={Medical \& Biological Engineering \& Computing},
  pages={1--13},
  year={2022},
  publisher={Springer}
}

@article{mountney2010three,
  title={Three-dimensional tissue deformation recovery and tracking},
  author={Mountney, Peter and Stoyanov, Danail and Yang, Guang-Zhong},
  journal={IEEE Signal Processing Magazine},
  volume={27},
  number={4},
  pages={14--24},
  year={2010},
  publisher={IEEE}
}

@article{azagra2022endomapper,
  title={EndoMapper dataset of complete calibrated endoscopy procedures},
  author={Azagra, Pablo and Sostres, Carlos and Ferrandez, {\'A}ngel and Riazuelo, Luis and Tomasini, Clara and Barbed, Oscar Le{\'o}n and Morlana, Javier and Recasens, David and Batlle, Victor M and G{\'o}mez-Rodr{\'\i}guez, Juan J and others},
  journal={arXiv preprint arXiv:2204.14240},
  year={2022}
}

